Culture Clash: When Deceptive Design Meets Diverse Player Expectations

Deceptive game designs that manipulate players are increasingly common in the gaming industry, but the impact on players is not well studied. While studies have revealed player frustration, there is a gap in understanding how cultural attributes affect the impact of deceptive design in games. This paper proposes a new research direction on the connection between the representation of culture in games and player response to deceptive designs. We believe that understanding the interplay between cultural attributes and deceptive design can inform the creation of games that are ethical and entertaining for players around the globe.

==> 04-Conclusion.tex <==
%\hilda{I don't think we need a standalone conclusion given the page limit.}
%In conclusion, while the HCI research community are paying more and more attention on deceptive design in games, the role of cultural attributes has been neglected. While literature showed that cultural attributes can enrich the gaming experience, our Genshin Impact example demonstrates their potential for facilitating deceptive game design. Our work suggests a necessity to explore this interplay between cultural attributes and the impacts of deceptive game design on players. We proposed three possible research directions that can achieve the thorough understanding of this interplay. 

==> Note.tex <==
Similarly, in ``Super Smash brothers: Ultimate'', character naming conventions differ between Japanese and English, with the former adding additional context in the character's names; the character Olimar is simply named "Olimar" in English, while the Japanese name translates to ``Pikmin and Olimar'', emphasizing Olimar's use of `Pikmin' as weapons.


Animal Crossing has time-gated content and premium currency, with japanese culture. should be studied if we expand on this. The VR version of it 
